Online Temporal Fusion for Vectorized Map Construction in Mapless Autonomous Driving

To reduce the reliance on high-definition (HD) maps, a growing trend in autonomous driving is leveraging onboard sensors to generate vectorized maps online. However, current methods are mostly constrained by processing only single-frame inputs, which hampers their robustness and effectiveness in complex scenarios. To overcome this problem, we propose an online map construction system that exploits the long-term temporal information to build a consistent vectorized map. First, the system efficiently fuses all historical road marking detections from an off-the-shelf network into a semantic voxel map, which is implemented using a hashing-based strategy to exploit the sparsity of road elements. Then reliable voxels are found by examining the fused information and incrementally clustered into an instance-level representation of road markings. Finally, the system incorporates domain knowledge to estimate the geometric and topological structures of roads, which can be directly consumed by the planning and control (PnC) module. Through experiments conducted in complicated urban environments, we have demonstrated that the output of our system is more consistent and accurate than the network output by a large margin and can be effectively used in a closed-loop autonomous driving system.

==> fig/fig_lanejuction.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth,trim={0 0.1cm 0 0},clip]{fig/figures/SLM-topo_ex.pdf}
\caption{A closed-loop test of our autonomous vehicle in the split scenario. The black numbers and arrows indicate different lanes and their linkages. The PnC module was able to perform a smooth lane change based on the road information from our method.}
\label{fig_ex_lanejuction}
\end{figure}

==> fig/fig_time.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth,trim={0 0.2cm 0 0},clip]{fig/figures/SLM-time3.pdf}
\caption{Runtime on the NVIDIA DRIVE Orin platform.}
\label{fig_time}
\end{figure}

==> sec/6_acknowledgement.tex <==
\section*{ACKNOWLEDGMENT}

The preferred spelling of the word ÒacknowledgmentÓ in America is without an ÒeÓ after the ÒgÓ. Avoid the stilted expression, ÒOne of us (R. B. G.) thanks . . .Ó  Instead, try ÒR. B. G. thanksÓ. Put sponsor acknowledgments in the unnumbered footnote on the first page.
